Simple Methods to Represent Shapes with Sample Spheres

Representing complex shapes with simple primitives in high accuracy is important for a variety of applications in computer graphics and geometry processing. Existing solutions may produce suboptimal samples or are complex to implement. We present methods to approximate given shapes with user-tunable number of spheres to balance between accuracy and simplicity: touching medial/scale-axis polar balls and k-means smallest enclosing circles. Our methods are easy to implement, run efficiently, and can approach quality similar to manual construction.

==> Makefile <==
DRAFT = draft
FINAL = final
QUICK = quick

ROOT_BIB_SOURCES = ../doc/paper.bib ../doc/misc.bib
BIB_SOURCES = filtered.bib

PAPER_SOURCES := $(wildcard *.tex)
DRAFT_SOURCES = draft.tex $(PAPER_SOURCES)
FINAL_SOURCES = final.tex $(PAPER_SOURCES)
QUICK_SOURCES = quick.tex $(PAPER_SOURCES)

VECTOR_DIR = figs/vector/
RASTER_DIR = figs/raster/
VECTOR_FIGS = 
SVG_FIGS := $(wildcard $(VECTOR_DIR)/*.svg) $(wildcard $(RASTER_DIR)/*.svg)

RASTER_FIGS = #$(RASTER_DIR)/161.jpg

VECTOR_EPS = $(VECTOR_FIGS:.fig=.eps)
VECTOR_PDF = $(VECTOR_EPS:.eps=.pdf)
SVG_PDF = $(SVG_FIGS:.svg=.pdf)

ALL_FIGS = $(VECTOR_FIGS) $(RASTER_FIGS) $(SVG_PDF)

all: quick draft final

draft: $(DRAFT).pdf
final: $(FINAL).pdf
quick: $(QUICK).pdf

%.ps : %.fig
	fig2dev -L ps -c $< > $@

# fig2eps is nice, you can download it from
# http://soliton.science.uva.nl/~kager/figepspdf/fig2eps.htm
%.eps : %.fig
	 ./fig2eps -f $<

%.pdfnoembed : %.eps
	 epstopdf $< --outfile $@

%.pdf : %.pdfnoembed
	ps2pdf13 -dPDFSETTINGS=/prepress $< $@

%.pdf : %.svg
	inkscape $< --export-pdf $@

$(BIB_SOURCES) : $(ROOT_BIB_SOURCES)
	echo "% Automatically generated file, do not edit!" > $@
	sed -e 's/doi\s*=/_doi =/gI' -e 's/url\s*=/_url =/gI' -e 's/issn\s*=/_issn =/gI'  -e 's/isbn\s*=/_isbn =/gI'  -e 's/month\s*=/_month =/gI' $^ >> $@

$(DRAFT).pdf : $(DRAFT_SOURCES) $(ALL_FIGS) $(DRAFT).bbl
	pdflatex $(DRAFT)

$(DRAFT).aux : $(DRAFT_SOURCES) $(ALL_FIGS)
	pdflatex $(DRAFT)

$(DRAFT).bbl : $(DRAFT_SOURCES) $(BIB_SOURCES) $(DRAFT).aux 
	bibtex $(DRAFT)

$(FINAL).pdf : $(FINAL_SOURCES) $(ALL_FIGS) $(FINAL).bbl
	pdflatex $(FINAL)

$(FINAL).aux : $(FINAL_SOURCES) $(ALL_FIGS)
	pdflatex $(FINAL)

$(FINAL).bbl : $(FINAL_SOURCES) $(BIB_SOURCES) $(FINAL).aux 
	bibtex $(FINAL)

$(QUICK).pdf : $(QUICK_SOURCES) $(ALL_FIGS) $(QUICK).bbl
	pdflatex $(QUICK)

$(QUICK).aux : $(QUICK_SOURCES) $(ALL_FIGS)
	pdflatex $(QUICK)

$(QUICK).bbl : $(QUICK_SOURCES) $(BIB_SOURCES) $(QUICK).aux 
	bibtex $(QUICK)

clean:
	rm -f *.pdf *.out *.dvi *.bbl *.aux *.blg *.log $(SVG_PDF)

